TempLM: Distilling Language Models into Template-Based Generators

While pretrained language models (PLMs) have greatly improved text generation, they have also been known to produce unfaithful or inappropriate content. In contrast, classic template-based systems provide strong guarantees of faithfulness at the cost of fluency. We propose TempLM, which achieves the best of both worlds by distilling a PLM into a template-based generator. On the E2E and SynthBio data-to-text datasets, we show that TempLM is more faithful than the original PLM and is more fluent than prior template systems. Notably, on an out-of-domain evaluation, TempLM reduces a finetuned BART model's unfaithfulness rate from 83% to 0%. In a human study, we find that TempLM's templates substantially improve upon human-written ones in BERTScore.

==> Makefile <==
TEXTIDOTE_VERSION := $(shell textidote --version 2>/dev/null)
IGNORE_RULES="sh:c:noin,lt:en:MORFOLOGIK_RULE_EN_US,lt:en:EN_UNPAIRED_BRACKETS,lt:en:CURRENCY,lt:en:PUNCTUATION_PARAGRAPH_END,sh:seclen"

main.pdf: clean
	latexmk -pdf main 2>&1 | awk 'BEGIN{IGNORECASE=1}/warning|!/,/^$$/;'

update:
	cd tex-common && git pull

clean:
	rm main.pdf *.aux *.bbl *.blg *.dvi *.fdb_latexmk *.fls *.log || true

linter:
	chktex -l .chktexrc -V  main.tex

spell:
	./.githooks/spelling.sh .

textidote.jar:
	wget "https://github.com/sylvainhalle/textidote/releases/download/v0.8.1/textidote.jar"

style: textidote.jar
	java -jar textidote.jar --check en --ignore ${IGNORE_RULES} --output singleline main.tex

fullstyle: textidote.jar
	java -jar textidote.jar --check en --ignore ${IGNORE_RULES} --output plain main.tex

emacs:
	emacs --batch -l ~/.emacs --eval "(TeX-auto-generate \"tex-common/macros.sty\" \"auto\")"

makereview:
	git checkout -b reviewed && git push --set-upstream origin reviewed


==> figures/Qualitative.tex <==
\colorbox[rgb]{1.0,1.0,1.0}{\strut [name] }
\colorbox[rgb]{0.974,0.87,0.87}{\strut [be] }
\colorbox[rgb]{0.968,0.84,0.84}{\strut born }
\colorbox[rgb]{0.988,0.94,0.94}{\strut on }
% \colorbox[rgb]{0.998,0.99,0.99}{\strut [birth\_date\_month] [birth\_date\_day], [birth\_date\_year] in [birth\_place]}
\colorbox[rgb]{0.998,0.99,0.99}{\strut [birth\_date\_month]}
\colorbox[rgb]{1.0,1.0,1.0}{\strut [birth\_date\_day] }
\colorbox[rgb]{0.998,0.99,0.99}{\strut , }
\colorbox[rgb]{1.0,1.0,1.0}{\strut [birth\_date\_year] }
\colorbox[rgb]{0.998,0.99,0.99}{\strut in }
\colorbox[rgb]{0.996,0.98,0.98}{\strut [birth\_place] }
\bigg(~\dual{
% \colorbox[rgb]{0.8,0.0,0.0}{\strut , }
\colorbox[rgb]{0.8,0.0,0.0}{\strut {\color[rgb]{0.95,0.95,0.95}, south korea}}
% \colorbox[rgb]{0.858,0.29000000000000004,0.29000000000000004}{\strut korea }
/
\colorbox[rgb]{0.71,0.942,0.71}{\strut . [pronoun\_a] [be] born }
}~\bigg)
\colorbox[rgb]{0.966,0.83,0.83}{\strut to }
\colorbox[rgb]{0.964,0.82,0.82}{\strut [father] }
\colorbox[rgb]{0.964,0.82,0.82}{\strut and }
\colorbox[rgb]{0.99,0.95,0.95}{\strut [mother] }
\colorbox[rgb]{0.986,0.93,0.93}{\strut . }
\colorbox[rgb]{0.97,0.85,0.85}{\strut [pronoun\_a] }
\colorbox[rgb]{0.964,0.82,0.82}{\strut attended }
\colorbox[rgb]{0.942,0.71,0.71}{\strut the }
\colorbox[rgb]{0.982,0.91,0.91}{\strut [alma\_mater] }
\colorbox[rgb]{0.9179999999999999,0.59,0.59}{\strut and }
\colorbox[rgb]{0.862,0.31000000000000005,0.31000000000000005}{\strut worked }
\colorbox[rgb]{0.982,0.91,0.91}{\strut as }
\colorbox[rgb]{0.99,0.95,0.95}{\strut [article] }
\colorbox[rgb]{0.99,0.95,0.95}{\strut [occupation] }
\colorbox[rgb]{0.966,0.83,0.83}{\strut . }
\colorbox[rgb]{0.954,0.77,0.77}{\strut [pronoun\_a] }
\colorbox[rgb]{0.968,0.84,0.84}{\strut [be] }
\colorbox[rgb]{0.934,0.67,0.67}{\strut known }
\colorbox[rgb]{0.998,0.99,0.99}{\strut for }
\colorbox[rgb]{0.988,0.94,0.94}{\strut [known\_for] }
\colorbox[rgb]{0.926,0.63,0.63}{\strut and }
\colorbox[rgb]{0.88,0.4,0.4}{\strut [pronoun\_c] }
\colorbox[rgb]{0.934,0.67,0.67}{\strut codename}
\colorbox[rgb]{0.996,0.98,0.98}{\strut [be] }
\colorbox[rgb]{0.994,0.97,0.97}{\strut [codename] }
\colorbox[rgb]{0.978,0.89,0.89}{\strut . }
\colorbox[rgb]{0.966,0.83,0.83}{\strut [pronoun\_a] }
\colorbox[rgb]{0.9,0.5,0.5}{\strut worked }
\colorbox[rgb]{0.978,0.89,0.89}{\strut for }
\colorbox[rgb]{0.966,0.83,0.83}{\strut the }
\colorbox[rgb]{0.976,0.88,0.88}{\strut [agency] }
\colorbox[rgb]{0.958,0.79,0.79}{\strut and }
\colorbox[rgb]{0.91,0.55,0.55}{\strut [pronoun\_c] }
\colorbox[rgb]{0.944,0.72,0.72}{\strut operation }
\colorbox[rgb]{0.994,0.97,0.97}{\strut [be] }
\colorbox[rgb]{0.956,0.78,0.78}{\strut [operation] }
\colorbox[rgb]{0.9159999999999999,0.58,0.58}{\strut . }
\colorbox[rgb]{0.96,0.8,0.8}{\strut [pronoun\_a] }
\bigg(
\dual{
\colorbox[rgb]{0.8,0.0,0.0}{\strut {\color[rgb]{0.95,0.95,0.95}married} }
/
\colorbox[rgb]{0.71,0.942,0.71}{\strut was married }
}
\bigg)
\colorbox[rgb]{0.944,0.72,0.72}{\strut to }
\colorbox[rgb]{0.95,0.75,0.75}{\strut [partner] }
\colorbox[rgb]{0.9179999999999999,0.59,0.59}{\strut and }
\colorbox[rgb]{0.932,0.66,0.66}{\strut together }
\colorbox[rgb]{0.968,0.84,0.84}{\strut they }
\colorbox[rgb]{0.998,0.99,0.99}{\strut had }
\colorbox[rgb]{0.974,0.87,0.87}{\strut [number] }
\colorbox[rgb]{0.974,0.87,0.87}{\strut children }
\colorbox[rgb]{0.974,0.87,0.87}{\strut : }
\colorbox[rgb]{0.94,0.7,0.7}{\strut [children\_names] }
\colorbox[rgb]{0.964,0.82,0.82}{\strut . }
